Deep Learning for Koopman-based Dynamic Movement Primitives

The challenge of teaching robots to perform dexterous manipulation, dynamic locomotion, or whole--body manipulation from a small number of demonstrations is an important research field that has attracted interest from across the robotics community. In this work, we propose a novel approach by joining the theories of Koopman Operators and Dynamic Movement Primitives to Learning from Demonstration. Our approach, named \gls{admd}, projects nonlinear dynamical systems into linear latent spaces such that a solution reproduces the desired complex motion. Use of an autoencoder in our approach enables generalizability and scalability, while the constraint to a linear system attains interpretability. Our results are comparable to the Extended Dynamic Mode Decomposition on the LASA Handwriting dataset but with training on only a small fractions of the letters.

==> preamble.tex <==
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{tikz}
% \usepackage{lscape}
\usepackage{pdflscape}
\usepackage[acronym]{glossaries}
\usepackage{algorithm}
\usepackage{algpseudocode}

\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}

\renewcommand{\vec}{\mathbf}
\newcommand*{\vertbar}{\rule[-1ex]{0.5pt}{2.5ex}}
\let\oldref\ref
\renewcommand{\ref}[1]{(\oldref{#1})}

\def \encoder {\Phi}
\def \obs {\phi}
\def \decoder {\Psi}
\def \koop {K}

%%%%%% GLOSSARY %%%%%%
\setacronymstyle{long-short}
\newacronym{admd}{aDMD}{Autoencoder Dynamic Mode Decomposition}
\newacronym{dmd}{DMD}{Dynamic Mode Decomposition}
\newacronym{edmd}{eDMD}{Extended Dynamic Mode Decomposition}
\newacronym{lfd}{LfD}{Learning from Demonstration}
\newacronym{dmp}{DMP}{Dynamic Movement Primitives}
\newacronym{rl}{RL}{Reinforcement Learning}
\newacronym{lasa}{LASA}{Learning Algorithms and Systems Laboratory}
